TensorSLM: Energy-efficient Embedding Compression of Sub-billion Parameter Language Models on Low-end Devices

Small Language Models (SLMs, or on-device LMs) have significantly fewer parameters than Large Language Models (LLMs). They are typically deployed on low-end devices, like mobile phones and single-board computers. Unlike LLMs, which rely on increasing model size for better generalisation, SLMs designed for edge applications are expected to have adaptivity to the deployment environments and energy efficiency given the device battery life constraints, which are not addressed in datacenter-deployed LLMs. This paper addresses these two requirements by proposing a training-free token embedding compression approach using Tensor-Train Decomposition (TTD). Each pre-trained token embedding vector is converted into a lower-dimensional Matrix Product State (MPS). We comprehensively evaluate the extracted low-rank structures across compression ratio, language task performance, latency, and energy consumption on a typical low-end device, i.e. Raspberry Pi. Taking the sub-billion parameter versions of GPT-2/Cerebres-GPT and OPT models as examples, our approach achieves a comparable language task performance to the original model with around $2.0\times$ embedding layer compression, while the energy consumption of a single query drops by half.

==> sections/others/table.tex <==
\begin{table}[]\small
\caption{Parameters, number of floating-point operations (flops) of the compressed and uncompressed sub-billion models, latency on Raspberry Pi CPU. ``original'' means uncompressed model, $\texttt{PPL} \leq 100.0$ means the compressed model with negligible accuracy drop, and the notation $\varphi_{\text{max}}$ refers to the compressed model with maximum compression ratio. $l_{\text{text}}$ is the number of the tokens in the input text. (s/text, $l_{\text{text}}=50$)}\label{tab:exp-profile}
\centering
\begin{tabular}{l?lll?lll?lll}
\toprule
\multicolumn{1}{c?}{\multirow{2}{*}{\textbf{GPT Series}}} & \multicolumn{3}{c?}{\textbf{\# Params} (M)}                                          & \multicolumn{3}{c?}{\textbf{flops} ($l_{\text{text}}=100$)}    &  \multicolumn{3}{c}{\textbf{Raspberry Pi latency} }                      \\ \cline{2-10} 
\multicolumn{1}{c?}{}                                & \multicolumn{1}{l|}{original} & \multicolumn{1}{l|}{$\texttt{PPL}$} & $\varphi_{\text{max}}$ & \multicolumn{1}{l|}{original(G)} & \multicolumn{1}{l|}{$\texttt{PPL}$} & $\varphi_{\text{max}}$ & \multicolumn{1}{l|}{original} & \multicolumn{1}{l|}{$\texttt{PPL}$} & $\varphi_{\text{max}}$ \\ \midrule
 \multirow{4}{*}{GPT2} & \multicolumn{1}{l|}{81.9}         & \multicolumn{1}{l|}{67.06 }                  &    43.45      & \multicolumn{1}{l|}{20.25 G}         & \multicolumn{1}{l|}{$+$ 1.65 M}                  &    $+$ 0.13 M   & \multicolumn{1}{l|}{$0.19_{\pm 0.02}$}         & \multicolumn{1}{l|}{${0.36}_{\pm 0.19}$}                  &  $0.19_{\pm 0.03}$   \\ \cline{2-10}
 & \multicolumn{1}{l|}{124.44}         & \multicolumn{1}{l|}{106.36 }                  &   85.99       & \multicolumn{1}{l|}{40.49 G}         & \multicolumn{1}{l|}{$+$ 1.88 M}                  &   $+$ 0.13 M & \multicolumn{1}{l|}{$0.50_{\pm 0.19}$}         & \multicolumn{1}{l|}{${0.50}_{\pm 0.16}$}                  &  $0.71_{\pm 0.38}$ \\ \cline{2-10}
& \multicolumn{1}{l|}{354.82}         & \multicolumn{1}{l|}{326.45 }                  &  303.88         & \multicolumn{1}{l|}{142.25 G}         & \multicolumn{1}{l|}{$+$ 3.11 M}                  &     $+$ 0.20 M  & \multicolumn{1}{l|}{$1.23_{\pm 0.12}$}         & \multicolumn{1}{l|}{$1.26_{\pm 0.22}$ }                  &  $1.55_{\pm 0.36}$  \\ \cline{2-10}
 & \multicolumn{1}{l|}{774.03}         & \multicolumn{1}{l|}{734.28}                  &   710.83      & \multicolumn{1}{l|}{330.98 G}         & \multicolumn{1}{l|}{$+$ 2.30 M}                  &          $+$ 0.25 M 
 & \multicolumn{1}{l|}{$3.01_{\pm 0.47}$}         & \multicolumn{1}{l|}{$3.01_{\pm 0.29}$}                  &   $3.52_{\pm 0.44}$        
    \\ \midrule
 \multirow{3}{*}{CerebrasGPT} & \multicolumn{1}{l|}{111.05}         & \multicolumn{1}{l|}{101.78}                  &    71.87     & \multicolumn{1}{l|}{14.47 G}         & \multicolumn{1}{l|}{$+$ 0.38 M}     &$+$ 0.13 M   & \multicolumn{1}{l|}{$0.47_{\pm 0.21}$}  & \multicolumn{1}{l|}{$0.48_{\pm 0.23}$}                  & $0.72_{\pm 0.42}$              \\ \cline{2-10}
& \multicolumn{1}{l|}{255.98}         & \multicolumn{1}{l|}{226.69}                  &    200.59     & \multicolumn{1}{l|}{40.4 G}         & \multicolumn{1}{l|}{$+$ 1.63 M }                  &   $+$ 0.12 M  & \multicolumn{1}{l|}{$0.71_{\pm 0.02}$}         & \multicolumn{1}{l|}{$1.01_{\pm 0.29}$}   & $0.95_{\pm 0.27}$ \\ \cline{2-10}
 & \multicolumn{1}{l|}{590.31}         & \multicolumn{1}{l|}{543.45}                  &    511.07     & \multicolumn{1}{l|}{103.06 G}         & \multicolumn{1}{l|}{$+$ 2.30 M}                  &     $+$ 0.26 M & \multicolumn{1}{l|}{$1.81_{\pm 0.25}$}         & \multicolumn{1}{l|}{$1.89_{\pm 0.28}$}   &  $1.91_{\pm 0.24}$
         \\ \bottomrule

\end{tabular}
\end{table}
